GenTact Toolbox: A Computational Design Pipeline to Procedurally Generate Context-Driven 3D Printed Whole-Body Artificial Skins

Developing whole-body tactile skins for robots remains a challenging task, as existing solutions often prioritize modular, one-size-fits-all designs, which, while versatile, fail to account for the robot's specific shape and the unique demands of its operational context. In this work, we introduce GenTact Toolbox, a computational pipeline for creating versatile whole-body tactile skins tailored to both robot shape and application domain. Our method includes procedural mesh generation for conforming to a robot's topology, task-driven simulation to refine sensor distribution, and multi-material 3D printing for shape-agnostic fabrication. We validate our approach by creating and deploying six capacitive sensing skins on a Franka Research 3 robot arm in a human-robot interaction scenario. This work represents a shift from "one-size-fits-all" tactile sensors toward context-driven, highly adaptable designs that can be customized for a wide range of robotic systems and applications. The project website is available at https://hiro-group.ronc.one/gentacttoolbox

==> body/table/sensor_characteristics.tex <==
\begin{table*}[ht!]
    \vspace{1.5em}
    \centering
     %\renewcommand{\arraystretch}{0.5} % Increases row height
    \begin{tabular}{c c c c c c | c c c c c c}
        \toprule
        \multirow{2}{*}{\textbf{Skin Unit}} & \multirow{2}{*}{\textbf{Name}} & \multirow{2}{*}{\specialcell{\hfil \textbf{Nodules}\\ }} & \multirow{2}{*}{\specialcell{\textbf{Volume}\\\textbf{(\si{\centi\meter^3})}}} & \multirow{2}{*}{\specialcell{\hfil \textbf{Total R}\\\hfil\textbf{(\si{\kilo\ohm})}}} & \multirow{2}{*}{\specialcell{\textbf{Radius}\\ \textbf{Avg.} \textbf{(\si{\centi\meter})}}} & \multirow{2}{*}{\textbf{Skin Unit}}& \multirow{2}{*}{\textbf{Name}} & \multirow{2}{*}{\specialcell{\textbf{Nodules}\\ }} & \multirow{2}{*}{\specialcell{\textbf{Volume}\\\textbf{(\si{\centi\meter^3})}}} & \multirow{2}{*}{\specialcell{\textbf{Total R}\\\textbf{(\si{\kilo\ohm})}}} & \multirow{2}{*}{\specialcell{\textbf{Radius}\\ \textbf{Avg.} \textbf{(\si{\centi\meter})}}}\\[10pt] 
        \arrayrulecolor{black!30}\midrule

    %% ------------------------------------------------------
    %% Link 1 & 4
    %% ------------------------------------------------------
    \raisebox{-\totalheight}{\includegraphics[height=0.04\textwidth]{img/skinunits/pngs/link1.png}} & \multirow{4}{*}{Link 1} & \multirow{4}{*}{5} & \multirow{4}{*}{981.6} & \multirow{4}{*}{494.7} & \multirow{4}{*}{22.6} &  
    \raisebox{-\totalheight}{\includegraphics[height=0.04\textwidth]{img/skinunits/pngs/link4.png}} & \multirow{4}{*}{Link 4} & \multirow{4}{*}{4} & \multirow{4}{*}{656.7} & \multirow{4}{*}{428.7} & \multirow{4}{*}{21.2} \\

    %% ------------------------------------------------------
    %% Link 2 & 5
    %% ------------------------------------------------------

    \raisebox{-\totalheight}{\includegraphics[height=0.04\textwidth]{img/skinunits/pngs/link2.png}} & \multirow{4}{*}{Link 2} & \multirow{4}{*}{5} & \multirow{4}{*}{802.4} & \multirow{4}{*}{567.2} & \multirow{4}{*}{22.1} &  \raisebox{-\totalheight}{\includegraphics[height=0.035\textwidth]{img/skinunits/pngs/link5.png}} & \multirow{4}{*}{Link 5} & \multirow{4}{*}{6} & \multirow{4}{*}{884.1} & \multirow{4}{*}{177.3} & \multirow{4}{*}{24.7}\\

    %% ------------------------------------------------------
    %% Link 3 & 6
    %% ------------------------------------------------------


    \raisebox{-\totalheight}{\includegraphics[height=0.04\textwidth]{img/skinunits/pngs/link3.png}} & \multirow{4}{*}{Link 3} & \multirow{4}{*}{6} & \multirow{4}{*}{603.1} & \multirow{4}{*}{461.1} & 
    \multirow{4}{*}{20.1} & \raisebox{-\totalheight}{\includegraphics[height=0.04\textwidth]{img/skinunits/pngs/link6.png}} & \multirow{4}{*}{Link 6} & \multirow{4}{*}{4} & \multirow{4}{*}{366.0} & \multirow{4}{*}{100.6} & \multirow{4}{*}{9.4}\\

    
    \arrayrulecolor{black}\bottomrule
    \end{tabular}
    \caption{Sensor characterizations for the 6 skin units for the FR3. We list each skin unit's number of nodules, mesh volume, the total resistance of the conductive traces routed throughout the unit, and the average nodule radius.}
    \label{tab:sensor-characteristics}
\end{table*}



==> body/table/snr.tex <==
\begin{table}[t!]
% \renewcommand{\arraystretch}{1.5}
  \centering
  \begin{threeparttable}
  \small
  \begin{tabular}{
                  m{2cm} 
                  m{1.5cm}
                  m{1.5cm}
                  m{1.52cm}
                  }
\toprule
    \textbf{Skin Unit}
    & 
    \textbf{Trial 1}
    & 
   \textbf{Trial 2}
    & 
   \textbf{Trial 3}\\
     \arrayrulecolor{black!30}\midrule
    

     
    Link 1& 8 & 9 & 9 \\
    Link 2 & 28 & 28 & 28\\
    Link 3 & 371 & 428 & 395\\
    Link 4 & 33 & 35 & 33\\
    Link 5 & 20 & 14 & 22\\
    Link 6 & 594 & 561 & 455\\
\arrayrulecolor{black}\bottomrule

\end{tabular}
    \end{threeparttable}
  \caption{Signal-to-noise ratios (SNR) for each skin unit. The minimum SNR across all nodules is reported for each trial.}
  \label{tab:snr}
\end{table}

